Dropout Prediction over Weeks in MOOCs by Learning Representations of Clicks and Videos

This paper addresses a key challenge in MOOC dropout prediction, namely to build meaningful representations from clickstream data. While a variety of feature extraction techniques have been explored extensively for such purposes, to our knowledge, no prior works have explored modeling of educational content (e.g. video) and their correlation with the learner's behavior (e.g. clickstream) in this context. We bridge this gap by devising a method to learn representation for videos and the correlation between videos and clicks. The results indicate that modeling videos and their correlation with clicks bring statistically significant improvements in predicting dropout.

==> dfn.tex <==
\newtheorem{observation}{Observation}
\newtheorem{conjecture}{Conjecture}
\newtheorem{problem}{Problem}
\newtheorem{algo}{Algorithm}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
%\newtheorem{proof}{Proof}
\newtheorem{defi}{Definition}
\newcommand{\T}[1]{\boldsymbol{\mathscr{#1}}}   %% Tensor macro
\newcommand{\mb}[1]{\boldsymbol{\mathscr{#1}}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

% \newcommand{\method}{{\cal GigaTucker}\xspace}
\newcommand{\method}{\textsc{CMTF}\xspace}
\newcommand{\methodII}{\textsc{HaTuck2}\xspace}
\newcommand{\hide}[1]{}
\newcommand{\comment}[1]{{\tiny #1 }}
\newcommand{\semihide}[1]{{\tiny #1}}
%\newcommand{\reminder}[1]{{\em *** #1 ***}}
\newcommand{\reminder}[1]{{\textsf{\textcolor{red}{[#1]}}}}
\newcommand{\ukang}[1]{{\textsf{\textcolor{red}{[From U: #1]}}}}
\newcommand{\revise}[1]{\textcolor{BrickRed}{#1}}

\newcommand{\krp}[2]{ \left( \mathbf{#1}\odot\mathbf{#2} \right)}

\def\blambda{\mbox{\boldmath ${\lambda}$}}
\newcommand{\makeclean}{
    \renewcommand{\reminder}[1]{}
}

%\newcommand{\QED}{ \hfill {\bf QED}}
\newcommand{\tight}{ \setlength{\itemsep}{-1.0\itemsep} }
    % makes lists tighter

\newcommand{\tsection}[1]{ \vspace{-1.0\baselineskip} \section{#1} \vspace{-2mm} }
\newcommand{\tsubsection}[1]{ \vspace{-0.75\baselineskip} \subsection{#1} \vspace{-0.5\baselineskip} }

% naming conventions
\newcommand{\hadi}{{\cal HADI}\xspace}
\newcommand{\mapreduce}{\textsc{MapReduce}\xspace}
\newcommand{\hadoop}{\textsc{Hadoop}\xspace}

\newcommand{\PassA}{{\tt Stage1}\xspace}
\newcommand{\PassAMap}{{\tt Stage1-Map}\xspace}
\newcommand{\PassARed}{{\tt Stage1-Reduce}\xspace}
\newcommand{\PassB}{{\tt Stage2}\xspace}
\newcommand{\PassBMap}{{\tt Stage2-Map}\xspace}
\newcommand{\PassBRed}{{\tt Stage2-Reduce}\xspace}
\newcommand{\PassC}{{\tt Stage3}\xspace}
\newcommand{\PassCMap}{{\tt Stage3-Map}\xspace}
\newcommand{\PassCRed}{{\tt Stage3-Reduce}\xspace}

\newcommand{\diameter}{{\tt diameter}}
\newcommand{\npairs}{{\tt npairs}}
\newcommand{\gcc}{{\tt gcc}}
\newcommand{\entropy}{{\tt entropy}}
% \newcommand{\nedges}{{\tt nedges}}
\newcommand{\sv}{{\mbox{$\lambda_1$}}}
\newcommand{\avgd}{{\tt avgd}}

% math symbol definitions
\newcommand{\mat}[1]{{\bf{#1}}}
\newcommand{\nnodes}{N}     % number of nodes
\newcommand{\nedges}{E}     % number of edges
\newcommand{\deff}{{d_{eff}}}   % effective diameter
\newcommand{\Er}{{E_{r}}}   % number of retained edges
\newcommand{\Nr}{{N_{r}}}   % number of retained nodes
\newcommand{\Nc}{{N_c}}   % number of nodes at critical point
\newcommand{\Ec}{{E_c}}   % number of nodes at critical point
\newcommand{\Ngcc}{{N_{gcc}}} % number of nodes in gcc, at critical poing
\newcommand{\NPairc}{{N_{NPAIRS}}} % number of reachable pairs, at critical poing
\newcommand{\dc}{{d_{c}}} % diameter at critical point
\newcommand{\Lambdac}{{\lambda_{c}}} % First eigenvalue at critical point
% \newcommand{\RED}{ {\em RED } } % random edge deletion
% \newcommand{\FED}{ {\em FED } } % friendly edge deletion
% \newcommand{\HED}{ {\em HED } } % hostile edge deletion


\newcommand{\ben}{\begin{enumerate*}}
\newcommand{\een}{\end{enumerate*}}
\newcommand{\bit}{\begin{itemize*}}
\newcommand{\eit}{\end{itemize*}}

% shorthands
\newcommand{\citationsds}{{CITATIONS}}
\newcommand{\epinionsds}{{EPINIONS}}
\newcommand{\patentsds}{{PATENTS}}
\newcommand{\net}[1]{{\textsc{#1}}}

%\newcommand{\QED}{\hfill $\Box$ \hfill}
\newcommand{\model}{\textsc{CommunityConnection}}

